A Least-Privilege Memory Protection Model for Modern Hardware

We present a new least-privilege-based model of addressing on which to base memory management functionality in an OS for modern computers like phones or server-based accelerators. Existing software assumptions do not account for heterogeneous cores with different views of the address space, leading to the related problems of numerous security bugs in memory management code (for example programming IOMMUs), and an inability of mainstream OSes to securely manage the complete set of hardware resources on, say, a phone System-on-Chip. Our new work is based on a recent formal model of address translation hardware which views the machine as a configurable network of address spaces. We refine this to capture existing address translation hardware from modern SoCs and accelerators at a sufficiently fine granularity to model minimal rights both to access memory and configure translation hardware. We then build an executable specification in Haskell, which expresses the model and metadata structures in terms of partitioned capabilities. Finally, we show a fully functional implementation of the model in C created by extending the capability system of the Barrelfish research OS. Our evaluation shows that our unoptimized implementation has comparable (and in some cases) better performance than the Linux virtual memory system, despite both capturing all the functionality of modern hardware addressing and enabling least-privilege, decentralized authority to access physical memory and devices.

==> 60-related-work.tex <==
\section{Related work}
\label{sec:relatedwork}

\RA{what have other's done? Or does this go into background ?}



\RA{From the OSDI PAPER }


% virtual memory

Virtual memory has been around for decades providing a uniform address space 
abstraction to processes. Programming with multiple virtual address spaces has 
been proposed~\cite{ElHajj:2016:SPM} which required that the physical mappings 
do not change between different processors in the system. 
%
% scc / xeon phi
%
Many core appliances such as the Intel SCC or the Xeon Phi provide an x86-like 
environment integrated into the host system while acting as an independent 
compute environment which has a different view of the resources in the 
system~\cite{Achermann:2014:MPBT, Intel:2014:XeonPhi}. Each core of the Intel 
SCC for example can be configured which memory int can access through their 
respective lookup tables.

Cosh~\cite{Baumann:2014:CCO} 

% gpus
OpenCL's Shared Virtual Memory extends the global memory region into the host 
memory region using three different types~\cite{Khronos:2015:OpenCL}.
Similarly, nVidia's CUDA~\cite{nVidia:2013:UMCUDA} or HSA~\cite{HSA:2016:RPR} 
provide a unified view of memory. 

%hdsm

% iommus


% pgas 

% ndp
Data movement between DRAM and processors is costly and the gap between 
processors and DRAM speeds is growing, in memory processing or 
micro-controllers close to may mitigate certain 
limitations~\cite{Patterson:1997:CIR}. Processing data near memory or storage 
poses the question about proper OS abstractions~\cite{Barbalace:2017:TTO} and 
require a way to unambiguously refer to memory regardless of which module 
accesses it.

% genz

% device trees

% popcorn
Popcorn Linux~\cite{Barbalace:2015:PBP} provides a single system image 
abstraction to applications by making the processor islands transparent to the 
user. Popcorn Linux's support of software DSM was extended to support 
heterogeneous distributed shared memory to enable cross-ISA 
migration~\cite{Barbalace:2017:BBH}.

In DVMT~\cite{Alam:2017:DVM}, applications request physical frames from the OS 
that have specified properties. The system allows applications to customize how 
the virtual-to-physical mapping is set up by registering a TLB miss handler for 
the special DVMT range.

% other verified OSes
Other verified OSes do not tackle the problem of how memory accesses are routed 
through the system. CertiKOS~\cite{Gu:2016:CEA} proves functional correctness 
with the specification of the x86mc machine, a subset of standard x86, which 
models memory accesses to abstract regions of private, shared or atomic memory.
CertiKOS manages physical memory at the granularity of pages.
\RA{TODO: seL4}

% cbufs
The CBuf\cite{Ren:2016:CES} system globally manages virtual and physical memory 
focusing on efficient sharing and moving data between protection domains. CBuf 
unifies shared-memory, memory allocation and system-wide physical memory 
allocation.

DRAM channel and bank interleaving can cause slowdowns up to 
36\%~\cite{Hillenbrand:2017:MPM} due to interference, while partitioning limits 
the available bandwidth for a single application. Hillenbrand \etal 
in~\cite{Hillenbrand:2017:MPM} modify memory controller configurations of 
commodity hardware to provide DRAM aliases---a technique which effectively 
breaks the uniform view assumption.



%





ptasks\cite{Rossbach:2011:POS}

Specifying and dynamically verifying address translation-aware memory 
consistency\cite{Romanescu:2010:SDV}


\cite{Lindstrom:1995:GUT}




memory coherence \cite{Li:1989:MCS}



migration in heterogeneous systems\cite{DeVuyst:2012:EMH}

K2: a mobile operating system for heterogeneous coherence 
domains\cite{Lin:2014:KMO}



Mosaic: a GPU memory manager with application-transparent support for multiple 
page sizes\cite{Ausavarungnirun:2017:MGM}






The Scalable Heterogeneous Computing (SHOC) benchmark 
suite\cite{Danalis:2010:SHC}


VAST: the illusion of a large memory space for GPUs\cite{Lee:2014:VIL}

==> paper-commands.tex <==

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08emT\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

%\graphicspath{{./graphics/}}%helpful if your graphic files are in another directory


% COMMENTS
\ifisdraft
\usepackage[textsize=footnotesize]{todonotes}
\newcommand{\redcomment}[1]{\textcolor{red}{\textbf{#1}} }
\newcommand{\sidenote}[1]{\todo[linecolor=orange,backgroundcolor=yellow!25,bordercolor=orange]{#1}}
\newcommand{\camtodo}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{#1}}
\newcommand{\camdone}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green]{#1}}
\newcommand{\camready}[1]{\textcolor{green}{#1}}
\else
\newcommand{\sidenote}[1]{}
\newcommand{\redcomment}[1]{ }
\newcommand{\camtodo}[1]{ }
\newcommand{\camdone}[1]{ }
\newcommand{\camready}[1]{#1}
\fi

\newcommand{\RA}[1]{\redcomment{RA: #1}}
\newcommand{\DC}[1]{\redcomment{DC: #1}} 
\newcommand{\TR}[1]{\redcomment{TR: #1}} 

\newcommand{\ra}[1]{\sidenote{RA: #1}}
\newcommand{\dc}[1]{\sidenote{DC: #1}} 
\newcommand{\tr}[1]{\sidenote{TR: #1}}


==> paper-conference.tex <==
% Rights management information. 
% This information is sent to you when you complete the rights form.
% These commands have SAMPLE values in them; it is your responsibility as an author to replace
% the commands and values with those provided to you when you complete the rights form.
%
% These commands are for a PROCEEDINGS abstract or paper.
\copyrightyear{2020}
\acmYear{2020}
\setcopyright{acmlicensed}
\acmConference[ASPLOS'20]{ASPLOS'20: The 25th International Conference on Architectural Support for  Programming Languages and Operating Systems}{March 16-20, 2020}{Lausanne, Switzerland}
\acmBooktitle{ASPLOS'20: The 25th International Conference on Architectural Support for  Programming Languages and Operating Systems, March 16-20,  2020, Lausanne, Switzerland}
\acmPrice{0.00}
\acmDOI{}
\acmISBN{}
